Contact-less manipulation of millimeter-scale objects via ultrasonic levitation

Although general purpose robotic manipulators are becoming more capable at manipulating various objects, their ability to manipulate millimeter-scale objects are usually very limited. On the other hand, ultrasonic levitation devices have been shown to levitate a large range of small objects, from polystyrene balls to living organisms. By controlling the acoustic force fields, ultrasonic levitation devices can compensate for robot manipulator positioning uncertainty and control the grasping force exerted on the target object. The material agnostic nature of acoustic levitation devices and their ability to dexterously manipulate millimeter-scale objects make them appealing as a grasping mode for general purpose robots. In this work, we present an ultrasonic, contact-less manipulation device that can be attached to or picked up by any general purpose robotic arm, enabling millimeter-scale manipulation with little to no modification to the robot itself. This device is capable of performing the very first phase-controlled picking action on acoustically reflective surfaces. With the manipulator placed around the target object, the manipulator can grasp objects smaller in size than the robot's positioning uncertainty, trap the object to resist air currents during robot movement, and dexterously hold a small and fragile object, like a flower bud. Due to the contact-less nature of the ultrasound-based gripper, a camera positioned to look into the cylinder can inspect the object without occlusion, facilitating accurate visual feature extraction.

==> DesignSim.tex <==
\section{Design Simulation}
\label{Sec:DesignSim}


Prior to designing the second iteration, the first iteration design was simulated using a MATLAB model to explain the effect the petri dish has on the the object being trapped inside the acoustic device. In the MATLAB model of the acoustic field, it is important that the incident acoustic wave is modeled but also the reflected acoustic wave from the surface, the object initially rests on, needs to be modeled. By using the Gor'kov Potential and taking the gradient \textcolor{red}{[??? Add gorkov equation]} to compute the vertical force, we can better understand the effect the petri dish has on the acoustic pressure field, and lift force which allows the particle to be lifted further from the table.

In the first iteration case, the reflection due to the petri dish is also modeled as an acoustically reflective surface. Similar to the method of images used in electrostatics to express field flux lines, the reflected acoustic wave due to the table top surface is modeled as originating from an imaginary source located below the plane of reflection. Additionally, the same imaginary source model is applied to the petri dish reflector above the trap. Analogous to an optics situation, the bottom table surface and the top petri dish act as acoustic mirrors and like infinite parallel mirrors there reflections will seem to continue to infinite. However, when modeling each additional series of reflected imaginary sources, we see that with attenuation of the acoustic wave, only the first set of reflected sources need to be computed as additional series of imaginary sources result in no additional pressure magnitude change, \textcolor{red}{[!!! see acoustic mirroring figure]}.

Based on the mirrored sources simulation, the impact of the vertical petri dish movement can be approximated by real acoustic sources located 20mm above the first set of transducers applying a phase shift to represent the movement. Figure \textcolor{red}{[!!! See Figure of phase sim]} shows a side by side comparison of the vertical acoustic force field when moving the petri dish versus applying a phase shift to an upper ring of acoustic sources. The figure shows a minimal amount of difference to the center column of acoustic nodes thus motivating iteration 2's design.


